On The Problem of the Quantum Heterotic Vortex

We address the problem of non-Abelian super-QCD, with a Fayet-Iliopoulos term, as seen from the vortex worldsheet perspective. Together with the FI term $\xi$, also a mass $\mu$ for the adjoint superfield $\Phi$ enters in the game. This mass allows the interpolation between $\N=2$ and $\N=1$ super-QCD. While the phenomenology of the $\N=2$ case ($\mu=0$) is pretty much understood, much remains to be clarified for the finite-$\mu$ case. We distinguish, inside the parameter space spanned by the FI term and the mass $\mu$, four different corners where some quantitative statements can be made. These are the regions where the strong dynamics can, in some approximation, be quantitatively analyzed. We focus in particular on two questions: 1) Is the quantum vortex BPS or non-BPS? 2) What is the phase of the internal non-Abelian moduli? We find that the answer to these questions strongly depends upon the choice of the linear term in the superpotential. We also try to explain what happens in the most unexplored, and controversial, region of parameters, that of the quantum heterotic vortex, where $\Lambda \ll \sqrt{\xi} \ll \mu$.

==> z.tex <==

This Appendix contains more details about the fermionic zero modes. We focus in particula on the effect of the $\mu$ parameter. 


Zero modes for the Dirac equation are
\beq
(\lambda_R)^a_{\,b} =.. (1-f(r)) \  \bar\vp^a  {\xi}_{R \, b } 
\quad {\rm and } \quad 
(\psi_{q\,L})^a_{\,i} =.. (1-q(r)^2)  \  \vp^a  \bar{\xi}_{R \, i } 
\eeq
\beq
(\psi_L^{\0})^a_{\,b}= ..  (1-f(r))  \ \bar\vp^a  {\xi}_{L \, b } 
\quad {\rm and }\quad   
(\psi_{\tq \, R}^{\0})^a_{\,i} = .. ((1-q(r)^2) \   \vp^a  \bar{\xi}_{L \, i }
\eeq















We can use an expansion in powers of $\mu/\sqrt{\xi}$
$ \psi = (\psi_L^{\0},\psi_R^{\1})$ 

$ \psi_{\tq} = (\psi_{\tq \,L}^{\1} , \psi_{\tq \,R}^{\0} )$


\bea
-\frac{i}{g^2} \nabla_{z} \psi_R^{\1} - \sqrt{2}\bar{{\psi}}_{\tq \,L \, i}^{\1} {q}_i^{\dagger}  &=& \sqrt{2}  \mu  \bar{\psi}_L^{\0}
\nonumber \\
-i\nabla_{\bar{z}}\psi_{\tq \,L}^{\1} -\sqrt{2}q_i^{\dagger}\bar{\psi}_{R}^{\1} &=& 0 \ .
\label{nonsusyfermionsperturbed}
\eea




\beq
\psi_R^{\1}=    
\quad {\rm and }\quad
\psi_{\tq \, L}^{\1}= 0 
\eeq



\beq
\bar{\vp}_l \xi_{L}^{\1 l} = \mu \bar{\zeta}_L^{\0}
\eeq

From here the coefficient of proortionality in (\ref{etconjecture}) is 

